On the Privacy Risks of Deploying Recurrent Neural Networks in Machine Learning Models

We study the privacy implications of training recurrent neural networks (RNNs) with sensitive training datasets. Considering membership inference attacks (MIAs), which aim to infer whether or not specific data records have been used in training a given machine learning model, we provide empirical evidence that a neural network's architecture impacts its vulnerability to MIAs. In particular, we demonstrate that RNNs are subject to a higher attack accuracy than feed-forward neural network (FFNN) counterparts. Additionally, we study the effectiveness of two prominent mitigation methods for preempting MIAs, namely weight regularization and differential privacy. For the former, we empirically demonstrate that RNNs may only benefit from weight regularization marginally as opposed to FFNNs. For the latter, we find that enforcing differential privacy through either of the following two methods leads to a less favorable privacy-utility trade-off in RNNs than alternative FFNNs: (i) adding Gaussian noise to the gradients calculated during training as a part of the so-called DP-SGD algorithm and (ii) adding Gaussian noise to the trainable parameters as a part of a post-training mechanism that we propose. As a result, RNNs can also be less amenable to mitigation methods, bringing us to the conclusion that the privacy risks pertaining to the recurrent architecture are higher than the feed-forward counterparts.

==> PETS/tex/related_works.tex <==
\section{Related Works}

We first briefly review some known privacy and security risks of machine learning models. 
Machine learning models are known to be vulnerable to poisoning attacks which refer to perturbations or alterations in a training dataset such that the resulting model does not yield its intended behavior \cite{jagielski2018manipulating,mozaffari2014systematic}. 
Adversarial examples or evasion attacks aim to find edge-case data records such that the victim model's output to such records is suboptimal \cite{goodfellow2014explaining}
The above two attacks compromise the integrity of the model. We now review adversaries who compromise the data confidentiality in the training datasets.
Model inversion attacks \cite{10.1145/2810103.2813677} aim to estimate certain attributes of the training data or ideally reconstruct the training data by observing the model outputs.
Finally, MIAs aim to infer whether or not a given data record has been used to train a model, which is the focus of this work.

The idea of MIAs was first introduced by \cite{homer2008resolving} to determine whether or not an individual's record is within complex genomic DNA mixtures.
The work in \cite{Shokri_2017} later developed the first MIA that targets the training dataset of a machine learning model in classification tasks. 
The subsequent empirical works either enhanced the performance of the existing MIAs \citep{salem2018ml}, uncovered unknown vulnerabilities, such as the vulnerability of training datasets with correlated data to MIAs in \citep{gomrokchi2021did}, or expanded the application domain of MIAs to more sophisticated machine learning tasks \cite{melis2019exploiting,pan2019you,song2019auditing}. We refer the reader to \citep{hu2021membership} for a comprehensive literature study. 

The existing MIAs do not distinguish between the internal model of the victim. In fact, RNNs are known to be vulnerable to MIAs in natural language processing tasks \cite{song2019auditing,brendan2018learning,Ramaswamy2020TrainingPL}; however, these works do not compare RNNs with their feed-forward alternatives, which is the focus of this work. We use the MIA layouts and accuracy results from the earlier works to design the MIAs that we use in the experiments. 

We next review the related MIA studies in the reinforcement learning domain. \cite{pan2019you} developed the first MIA that targets deep reinforcement learning agents. However, the MIA infers the transition probabilities of the environment, while we target the agent itself. Concurrently with and independently of this paper, \cite{gomrokchi2021did} develop an MIA for deep reinforcement learning agents which, similar to our work, infers the membership of roll-out trajectories. The above work develops the MIA to study agents with correlated training datasets, whereas we develop the MIA to study the vulnerability of agents that deploy RNNs. Moreover, we use RNNs to process trajectories with arbitrary lengths and the MIA in \citep{gomrokchi2021did} truncates the trajectories. 

We now review the works that study defending machine learning models against MIAs. The defense methods either use regularization or noise-additive methods, or a combination thereof. Examples of regularization defense methods are $\ell_2$-regularization \citep{Shokri_2017}, dropout and model stacking \citep{salem2018ml}, and max-min game \citep{10.1145/3243734.3243855}.
The noise-additive methods inject an external noise to different attributes of the network to either directly mislead MIAs through adversarial examples \citep{hunt2018chiron,jia2019memguard}, or to enforce differential privacy \citep{rahman2018membership,abadi2016deep,ji2014differential}. 

Differential privacy defense methods are often the most effective against MIAs; however, in doing so, they typically degrade the utility of the model under protection \citep{carlini2019secret,jia2019memguard}. 
Based on the Moments-Accountant method developed in \cite{abadi2016deep}, the $\mathrm{DP\mbox{-}FedAvg}$ algorithm obfuscates the gradients used in updating the weights of the network to enforce differential privacy \cite{brendan2018learning,Ramaswamy2020TrainingPL}.
While such noisy-gradient methods yield acceptable privacy-utility trade-offs, it may not be feasible to alter the learning algorithm and an output-perturbation mechanism would be preferred.


Perturbing the output of machine learning models often requires adding noise to a probability vector, e.g., class predictions or action probabilities, for which we use the Dirichlet mechanism \cite{gohari2020privacy}.
The Dirichlet mechanism is a non-invasive privacy mechanism in the sense that it does not require access to the internal attributes of the protected network and only perturbs the output post training. Applications of the Dirichlet mechanism have been studied in load ensemble control \citep{hassan2021privacy}, constant function market makers \citep{Chitra2021DifferentialPI}, and policy synthesis in Markov decision processes \citep{gohari2020privacy}. To the best of our knowledge, we are the first to empirically study the Dirichlet mechanism's effectiveness in defending machine learning models against MIAs.
